Analysis of Petri Nets and Transition Systems

This paper describes a stand-alone, no-frills tool supporting the analysis of (labelled) place/transition Petri nets and the synthesis of labelled transition systems into Petri nets. It is implemented as a collection of independent, dedicated algorithms which have been designed to operate modularly, portably, extensibly, and efficiently.

==> eptcsdata.tex <==
\providecommand{\firstpage}{53}
\providecommand{\publicationstatus}{S. Knight, I. Lanese, A. Lluch Lafuente and H. T. Vieira (Eds.):\\ 8th Interaction and Concurrency Experience (ICE 2015)\\
EPTCS 189, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.189.6}{10.4204/EPTCS.189.6}}

